DeCon: Detecting Incorrect Assertions via Postconditions Generated by a Large Language Model

Recently, given the docstring for the target problem and the target function signature, large language models (LLMs) have been used not only to generate source code, but also to generate test cases, consisting of test inputs and assertions (e.g., in the form of checking an actual output against the expected output). However, as shown by our empirical study on assertions generated by four LLMs for the HumanEval benchmark, over 62% of the generated assertions are incorrect (i.e., failed on the ground-truth problem solution). To detect incorrect assertions (given the docstring and the target function signature along with a sample of example inputs and outputs), in this paper, we propose a new approach named DeCon to effectively detect incorrect assertions via LLM-generated postconditions for the target problem (a postcondition is a predicate that must always be true just after the execution of the ground-truth problem solution). Our approach requires a small set of I/O examples (i.e., a sample of example inputs and outputs) for the target problem (e.g., the I/O examples included in the docstring for a target problem in HumanEval). We use the given I/O examples to filter out those LLM-generated postconditions that are violated by at least one given I/O example. We then use the remaining postconditions to detect incorrect assertions as those assertions that violate at least one remaining postcondition. Experimental results show that DeCon can detect averagely more than 64% (63% and 65.5% detected by GPT-3.5 and GPT-4, respectively) incorrect assertions generated by four state-of-the-art LLMs, and DeCon can also improve the effectiveness of these LLMs in code generation by 4% in terms of Pass@1. In addition, although DeCon might filter out correct assertions, the fault-finding ability of the remaining correct assertions decreases only slightly.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> approach/benchmark.tex <==
\subsection{Benchmark: \wenwangbench{}}
\label{sec: benchmark}

In this section, we introduce a pragmatic benchmark of code generation named \wenwangbench{}.
We first introduce the construction of \wenwangbench{}, followed by the workflow of a verification platform for automatic evaluation.

\subsubsection{Benchmark Construction}

We construct the benchmark from recently-committed code on GitHub.
First, we sort all projects with successfully-executed CI by the number of stargazers descendingly and keep the top 1,000 projects with at least one new commit since January 1, 2022.
Next, we extract all collected functions in these projects from the database, then kept the ones that meet all the following conditions:

\begin{itemize}
    \item does not exist in \wenwangdataset{}
    \item is not a test or deprecated function
    \item with a function-level docstring in English
    \item with at least three lines of code in the function body
    \item with at least one test case collected during the CI execution, and the input\&output can be successfully deserialized with the \emph{dill} library
    \item can run successfully in the verification platform and passed the test cases
\end{itemize}

We adopt a series of works to improve the confidence and reliability of the benchmark.
For the collected functions, we remove them from the dataset, search in the dataset again using the docstring and function signature, and remove \emph{all} matched samples to ensure that there is no overlap between the benchmark and the dataset.
To simulate the practical scenario, we classify each collected function to a runnable level with the same approach in Section~\ref{sec.classify}, and control the proportion of each level for a similar distribution with the dataset.
% To reduce false positives during evaluation, for problems with only one test case, we manually mutated the input and ran the function to get the expected output through the verification platform, and appended the input/output pairs as the supplementary test cases.
When verifying the correctness of a function generated by models, our verification platform adds the $main$ function to the file to which the function belongs and runs the file. 
The input and output of test cases obtained through CI are run in the entire project environment. 
Therefore, to ensure that the verification platform can correctly verify the function generated by the model, we execute test cases separately at the file level and use the output as the output of the test cases in the benchmark.

Finally, we involve 230 functions from 43 projects in \wenwangbench{}.
The right part of Figure~\ref{fig.run_dep_res} shows the distribution of runnable levels on \wenwangbench{}.
Besides the internal, contextual, and meta information, each function also contains supplementary test cases. The average number of test cases for each function in \wenwangbench{} is 10.34, and more than 73\% of functions have more than one test case in the benchmark.

% Even though the average test case for each function is not low, there are some functions with only 1 or 2 test cases. 
% In the future, we will try to supplement more than five test cases for each function in \wenwangbench{}.
% According to the functions in the newly submitted files after January 1, 2022 based on commit\_time, we obtained a total of 152 open source projects configured with Tox CI. A total of 8700 newly submitted functions were obtained from these open source projects, of which 5429 were functions with docstring. 
% Our criterion for judging whether a function is a newly submitted function is based on the module + function signature as the unique identifier.
% The data items we collected in our benchmark totally contains docstring and test cases collected by CI. 
% To expand the number of functions in our benchmark, we also collected 140 functions in the newly submitted files after January 1, 2022 based on commit\_time, these 140 functions contain docstring, but do not contain test cases. 
% Since the benchmark requires supporting test cases, For functions without test cases, we use copilot to generate test cases for the functions. Then one of our author check the test cases generated by copilot manually and finally expand 36 functions.

% To make our benchmark can validate the function with multiple runnable level, we also classify the data in our benchmark into six runnable level: self\_contained, slib\_runnable, plib\_runnable, class\_runnable, file\_runnable, and others.
% We use the same technique of runnable classification for \wenwangdataset{} to classify the runnable level of a function in the \wenwangbench{}.
% We find the distribution runnable classification of \wenwangbench{} is similar with \wenwangdataset{}.


\subsubsection{Verification Platform}

Since \wenwangbench{} involves functions with contextual dependency and non-primitive types, we need a verification platform to provide a ready runtime environment to automatically run and verify the code generated by code generation models.

We base this platform on Docker, where we clone and set up environments for all 43 projects.
To avoid Python and library version conflicts, under each repository's root directory, we first use \emph{pyenv} to set the local Python version to the highest version specified in the CI configuration, then use \emph{venv} to create an individual virtual environment for the current project.
After that, we trigger the CI tool to install dependencies and set up the project before running tests.

With the environment ready and given a model to evaluate, the platform can automatically inject the solution it generates into the project code and invokes the function to compare the actual output with the expected output.
To invoke the target function correctly, we generate the entry point code to set up some necessary prerequisites (like initializing the object before calling a member function) and load the input/output data into memory via deserialization.
Given \emph{n} solutions generated by the model, the platform automatically replaces the original function with each of them to \emph{simulate} how the code generation and recommendation work in an actual IDE.
After the replacement, the entry point code will be started, and the running output (e.g., return values, exceptions, errors, and console output) will be captured.
If the function returns with no error and exception, the platform will compare the actual output with the expected output. Comparison results of all 230 tasks will be used to compute the Pass@K metric at the end of the evaluation.


% Compared with HumanEval, \wenwangbench{} has two main advantages: (1) The test object for \wenwangbench{} is the functions in realistic development scenarios, and the functions in \wenwangbench{} are mined from open source projects. (2) \wenwangbench{} not only supports functions that are valid for the object with basic type (e.g., int, float, str), but also supports the object with complex types. The functions with complex objects often belong to class-level, file-level and project-level runnable.
% To achieve the first advantage, we strictly mine functions that not appear in \wenwangdataset{}, and most of them are submitted after 2022 from GitHub, and use CI to collect their test cases.
% Since the object in functions in HumanEval's are basic types, it does not need to consider the validation of functions belong to class, file, and project-level. 
% To achieve the second advantage, we built a verification platform that supports class, file, and project level. Next, we will introduce the construction of \wenwangbench{}'s verification platform in detail.
% To achieve the accuracy of the functions for verifying class-level dependencies, file-level dependencies, and project-level dependencies, we first need to serialize the input and output as objects of complex types and store them in the database in binary form. These stored data are then deserialized from the database into objects that can be executed in the program when testing functions that rely on objects of complex types. It is easy to serialize objects of complex types while the project is running, because all elements of serialization dependencies are available in the currently running project. At the same time, this requires that when deserializing the data stored in the database, it also needs to be executed in the entire project. Therefore, when verifying the correctness of functions in \wenwangbench{}, the verification platform of \wenwangbench{} needs the entire project where the function is located as the context.
% In the end, we selected 43 projects with a total of 230 functions for \wenwangbench{}.



% To verify the correctness of the functions in \wenwangbench{}, we need to automatically generate the correct calling function for each function. It should be noted that the calling function of dependent class-level executable functions is written inconsistently with other levels. Because the class level first instantiates the object of the class and other levels don't need to. 
% %Figures x and y show how calling functions are written at the class level and other levels.

% deserialize input and output of test cases, run and get, compare with

% Changed relative references in python files to absolute references
% Since there are relative references in the python file, the file cannot be run directly. And a large number of functions in our benchmark appear in python files where relative references exist. Therefore, we automatically change the relative reference in python to absolute reference.

% For each generated code to be tested, we replace the function location (in a file in a project) with the code in a python-compilable and executable format.
% Then execute the code in the project and determine whether the code is generated correctly according to whether the test cases are passed.


==> approach/dataset.tex <==
\subsection{Dataset: \wenwangdataset}
\label{sec: dataset}

In this section, we introduce the detailed collection of \wenwangdataset{}, including the selection of open-source projects, data collection, and further analysis.
A recent study~\cite{codex} shows that functions covered by tests are likely to be correct and well-written.
The core contribution of WenwangData is that all functions in WenwangData are covered by tests.

\subsubsection{Project Selection}

Following the Codex's way of collecting open-source data, we consider Python3-compatible GitHub repositories using Travis~\cite{travis} or Tox~\cite{tox} as the continuous integration (CI) system, which are the most popular CI tools for Python.
Specifically, we first search on GitHub for repositories with Python as the first primary programming language, then check whether there exist configuration files (travis.y(a)ml, tox.ini) under the repository root to determine whether this project uses Travis or Tox. For projects that use Travis and Tox, we further open the configuration file and check the target Python version specified for testing to determine whether this project supports Python version 3.
Finally, by June of 2022, we collect a total of 136,446 repositories, 36,039 of which configure Travis and Tox at the same time.

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.2\textwidth]{figure/travis_tox.pdf}
% 	\caption{Distribution of Travis and Tox Projects}
% 	\label{fig: distribution_travis_tox}
%   \vspace*{-1ex}
% \end{figure}

\subsubsection{Data Collection}

For each selected project, we try to rerun the CI locally and collect the functions invoked during a successful CI execution as our dataset.
Similar to Codex, we consider these functions to be correctly implemented since they are directly or indirectly tested by the developer.
For each function, we collect the following information for later use:

\begin{itemize}
    \item Internal Info: the annotation, docstring, signature, and code snippet of the function
    % \item Contextual Info: the content of the source file in which the function resides, the input argument values and the output/return values (if exists). For data of non-primitive types, we used the \textit{dill} library to serialize the object in binary format
    \item Contextual Info: the content of the source file in which the function resides
    \item Meta Info: the location (project, file path, and line ranges) of the function, and the version control information (commit id, commit timestamp, and committer) of the most recent commit that touched the function
\end{itemize}

To efficiently collect functions covered by tests from a massive number of projects, there are three challenges: (1) automatically prepare the environment required by the CI tool and the project, (2) efficiently analyze such a massive number of projects, and (3) dynamically collect the above information during testing.
We tackle these challenges step by step: First, based on the Ubuntu+Travis docker image from DockerHub, we prepare a base environment and write a script to automatically clone the repository with \textit{Git}, install the correct Python version configured by the CI tool with \textit{pyenv}.
After installing the Python interpreter, the system injects a tracing function into the installed Python, which would capture and save the above information into a MongoDB database when running Python code from the project. Next, we deploy this docker image to 500 containers on a cloud computing cluster with \textit{Kubernetes} and trigger the system to continuously analyze the next project in a queue of tasks. In this way, we are able to analyze all projects in parallel in 350 hours.

To make \wenwangdataset{} more useful for generating non-standalone functions, we also provide oracle\_contextual (the types, variables, and APIs defined/imported that the original function body actually depends) and all\_contextual (all types, variables, and APIs defined/imported in the current file) information for \wenwangdataset{}.
\emph{oracle\_context} information can be used as part of the input to the model in the inference stage, to verify whether prompting the model with the oracle information can improve the performance. However, it is usually difficult for the model to know oracle information in advance, so \wenwangdataset{} also provides the \emph{all\_context} information, that is, all types, variables, and APIs defined/imported in the current file. 
\wenwangdataset{} can be used by the model in both the training and inference stages.

We removed the functions contained in HumanEval and CoderEval in WenwangData. In total, we collected 301,320 functions from all projects and filtered out those with no docstring, resulting in 103,541 functions as the final dataset.
Compared with Codex's dataset, we do not restrict the standalone functions or use a pre-trained model to filter the data to avoid bias in distribution and tight binding with specific models.
Besides, we additionally consider functions without output/return value and functions that involve data of user-defined types in the input/output.
Therefore, we believe it provides a more reasonable choice when fine-tuning pre-trained models toward the task of generating code beyond standalone functions.

\begin{figure}
	\centering
	\includegraphics[width=0.7\textwidth]{figure/datadis.pdf}
	\caption{Distribution of Functions with Runnable Level Classification in \wenwangdataset{}}
	\label{fig: distribution_wenwang}
  \vspace*{-1ex}
\end{figure}
Figure~\ref{fig: distribution_wenwang} shows the distribution of functions with runnable level classification in \wenwangdataset{}.
We use the same definition and technique of runnable level classification as Yu et al~\cite{yu2023ce}.
The proportion of non-standalone functions in \wenwangdataset{} is 83\%.
The core contribution of \wenwangdataset{} is that all functions in \wenwangdataset{} are covered by tests.




% Similar with CoderEval, we also do several data augmentations for each function in 
% \subsubsection{Data Augmentation}
% \label{sec.classify}

% To better understand the task of pragmatic code generation, we additionally classify the dataset into different \textit{runnable levels} according to the \textit{contextual dependency} of functions.


% \paragraph{Contextual Dependency Identification}
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
% \begin{table*}[t]
% \caption{Contextual Dependency Types}
%     \centering
%     \footnotesize
%     \renewcommand{\arraystretch}{1.5}
%     \vspace*{-1.5ex}
%     \begin{tabular}{llll}
%     \toprule
%     Database Schema & \multicolumn{1}{c}{Dependency Type} & \multicolumn{1}{c}{Explanation} & \multicolumn{1}{c}{Example} \\ 
%     \midrule
%     \multirow{6}{*}{\makecell[l]{dependency: \{ \\
%     \hspace{\parindent} builtin: boolean, \\
%     \hspace{\parindent} standard\_lib: boolean, \\
%     \hspace{\parindent} public\_lib: boolean, \\
%     \hspace{\parindent} current\_class: boolean, \\
%     \hspace{\parindent} current\_file: boolean, \\
%     \hspace{\parindent} current\_project: boolean  \\
% \} }} & builtin & Python builtin types and functions, no need to import. & min(), round(), print() \\
%      & standard\_lib & Python standard libraries/modules, no need to install. & os, subprocess, sys \\
%      & public\_lib & Publicly available libraries on pypi.org, pip install first. & unittest2, requests, urllib \\
%      & current\_class & Code outside the function but inside the parent class. & self.xxx, self.f(), X.f() \\
%      & current\_file & Code outside the parent class but inside the current file. & func(), URL, name \\
%      & current\_project & Code in the other source files of the current project. & superclass (defined in anther file) \\
%      \bottomrule
%     \end{tabular}
    
%     \label{tab: run_dep_cla}
% \end{table*}
% We denote the context code elements that a function directly requires to run as its contextual dependency, which includes language-builtins, standard libraries, third-party public libraries, and code outside the function but within the current class, file, or project.
% Table~\ref{tab: run_dep_cla} shows the definition and exemplary explanation for each dependency type in Python code.
% For each entry in the database, we use a field named \textit{dependency} to store the identified dependencies.





% % Figure~\ref{fig: run_dep_imp} shows how we identified the contextual dependency of a function through program analysis on the whole project.
% We identify the contextual dependency of a function through program analysis on the whole project.
% Before the analysis, we first need to build a knowledge base that helps distinguish the references of Python-builtins, and the imports of standard or public libraries from the project-specific code.
% To do this, we cache all built-in types/functions/variables/constants and standard library names for each Python version from 3.0.0 to 3.10.0, as well as all public-available libraries on pypi.org.
% With this knowledge base, given a function to analyze, we retrieve the database to get the source file that it came from, then parse it to get a list of defined types/functions/variables/constants.
% For each dependency type, the criterion for setting it to true was whether the function \textit{used} the code of this type.
% For example, for a member function in a class, if it invokes a builtin function \lstinline{sorted()} to manipulate a member variable \lstinline{self.x}, we set the \lstinline{builtin} and \lstinline{current_class} to true.

% % \begin{figure*}
% % 	\centering
% % 	\includegraphics[width=0.7\textwidth]{figure/runnable_classifcation.png}
% % 	\caption{The Overview of Runtime Dependency Classification}
% % 	\label{fig: run_dep_imp}
% % \end{figure*}


% \paragraph{Runnable-level Classification}
% \begin{table}[t]
% \begin{threeparttable}
%     \centering
%     \setlength\tabcolsep{1.1pt}
%     \footnotesize
%     \renewcommand{\arraystretch}{1.2}
%     \caption{Matrix to Classify Runnable Level by Dependency}
%     \vspace*{-1.5ex}
%     \label{tab: run_dep_rdc}
%     \begin{tabular}{@{} ccccccccc @{}} % suppress vertical whitespace at start and end
%         \toprule
%         \diagbox[width=\dimexpr \textwidth/6+2\tabcolsep\relax, height=0.8cm]{ Runnable Level }{Dependency}
%         & \makecell{language \\ builtin} & \makecell{standard \\ library} & \makecell{public \\ library} & \makecell{current \\ class} & \makecell{current \\ file} & \makecell{current \\ project} \\
%         \midrule
%         self\_contained & $\bigcirc$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
%         \midrule
%         slib\_runnable & $\bigcirc$ & $\checkmark$ & $\times$ & $\times$ & $\times$ & $\times$ \\
%         \midrule
%         plib\_runnable & $\bigcirc$ & $\bigcirc$ & $\checkmark$ & $\times$ & $\times$ & $\times$ \\
%         \midrule
%         class\_runnable & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\checkmark$ & $\times$ & $\times$ \\
%         \midrule
%         file\_runnable & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\checkmark$ & $\times$ \\
%         \midrule
%         project\_runnable & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\checkmark$ \\
%         \bottomrule
%     \end{tabular}
%     \emph{\footnotesize
%         $\checkmark$ means true, $\times$ means false, and $\bigcirc$ means true/false.
%     }
%     \vspace*{-2.5ex}
%     \end{threeparttable}
% \end{table}
% According to the identified dependency, we classify the data into six levels, each of which indicates the minimal context scope that a function requires to run.
% The motivation is to simulate different scenarios of pragmatic code generation, analyze the advantage and shortcomings of existing models in more detail, and optimize them more systematically.


% We define a \textit{Dependency Matrix} for the classification, as shown in Table~\ref{tab: run_dep_rdc}.
% In this matrix, the row represents the runnable level, the column represents the dependency type, and each cell indicates whether the level of the row could depend on the dependency type of the column.
% From top to bottom, we define six levels from self\_contained to project\_runnable. Each level indicates the \emph{minimal} context scope a function requires to run.
% For example, plib\_runnable means the function \emph{at most} depends on public libraries,so it can run successfully outside the current source file and project, as long as the required Python version is satisfied and the libraries are installed.
% Note that we determine the runnable level by what it \emph{cannot} depend on, so the higher level wraps the lower levels (see Figure~\ref{fig.run_dep_res}), because intuitively if a function of the lower level can within its scope (say with standard library imports), it can also run given a larger scope (say the current file).



% The left part of Figure~\ref{fig.run_dep_res} shows the distribution of runnable levels on \wenwangdataset{}.
% Most (84\%) of the collected functions are file\_runnable, which indicates that the context information in the current file is necessary and critical for a code generation model to generate the function correctly.
% The class\_runnable functions account for half (54\%) of all functions, which is not surprising considering the prevalence of object-oriented programming in realistic and non-trivial projects.
% On the contrary, slib\_runnable only accounts for 17\% in our dataset but 100\% in the Codex dataset and the HumanEval benchmark. This fact proves the bias and mismatching in the model optimization and evaluation process with HumanEval, especially in the pragmatic generation of code in realistic settings.

% \begin{figure}
% 	\centering
% 	\includegraphics[width=1.0\linewidth]{figure/dis.pdf}
% 	\caption{Distribution of Runnable Level Classification}
% 	\label{fig.run_dep_res}
% \end{figure}


% --------------------------BACKUPS--------------------------

% First, we reproduced the CI environment of each project locally in docker instances, then injected a tracing function in the environment, which would capture the input, output, invocation location, and context code for each function invoked during integration testing. After that, the CI script was triggered and the data of invoked functions were recorded into a database. We further clustered the collected data into 4 groups, according to the external contextual information (dependencies) that a function requires to run. That is, functions depending on Python-builtin objects, Python-standard libraries, Pypi-public libraries, and the class. We expect this variety could enable the generation of different function types, e.g., self-contained, module, member or class functions. After filtering for maximum model input length, 49K examples are retained for fine-tuning.



% To implement the technique of runtime dependency classification, we first record all python build\_in type functions (e.g., $open$, $sorted$ ...), these functions can be executed directly in the python environment without any import.
% Then we record all the standard libraries in python (e.g., $os$, $subprocess$, $sys$), the functions belong to the standard libraries can directly import the library in the python environment and be executed successfully.
% Next we record the public libraries (e.g., $numpy$, $tensorflow$, $torch$) in python according to the download frequency. 
% Functions belong to the public libraries need to pip install the public library and import the public library in the python environment to execute successfully.
% After completing the above pre-recording, we analyze the dependencies of each level.
% Specifically, given any function to be classified and its file, we first analyze all functions and variables defined in the class or file where the function to be classified belong to.
% % After the preceding analysis, we get  
% Then we perform six dependency level analysis: Python Buildins, StandardLib, PublicLib, Class, File, and Project.



% \subsubsection{Competitive Programming Data}
% The following two datasets often provide dozens of successful code completions for each problem. Therefore, we can upsample each dataset by pairing up to five solutions with each problem description to avail the model of different correct solutions for the same problem specification. APPS~\cite{hendycks-etal-2021-apps} was proposed to benchmark the programming capability of code-generating models. It includes 10,000 programming tasks (5,000 train, 5,000 test) that require code generation/completion given a detailed problem description\footnote{\url{https://github.com/hendrycks/apps}}. Program arguments are provided from standard input as well as function calls, sometimes embedded inside the class. We use the train and test set programs, which we filter for the maximum input length of the model (1,024), retaining 43K examples. Code Contests (CC) is a similar dataset~\cite{alpha_code} for training and evaluation of competition-level code generation\footnote{\url{https://github.com/deepmind/code_contests}}, containing over 13K programming problems. After upsampling and length filtering, we retain 18K instances for fine-tuning.


% To build a dataset suitable for multiple application scenarios (such as competitive programming, realistic development), we construct the \wenwangdataset{} with multiple runnable level.
% To construct the \wenwangdataset{} with multiple runnable level, we first make a runtime dependency classification for each function in the \wenwangdataset{}. 
% \begin{figure*}
% 	\centering
% 	\includegraphics[width=0.7\textwidth]{figure/runnable_classify.png}
% 	\caption{Runtime Dependency Classification}
% 	\label{fig: run_dep_cla}
% \end{figure*}

% \begin{figure*}
% 	\centering
% 	\includegraphics[width=0.7\textwidth]{figure/runnable_count.png}
% 	\caption{Runnable Classification}
% 	\label{fig: run_dep_rdc}
% \end{figure*}
% We further clustered the collected data into 4 groups, according to the external contextual information (dependencies) that a function requires to run. That is, functions depending on the Python-builtin objects, the Python-standard libraries, the Pypi-public libraries, and the  class. We expect this variety would enable the generation of different function types, e.g., self-contained, module, member or class functions. After filtering for maximum model input length, 49K examples are retained for fine-tuning.

% \subsection{Sub-Runnable Open Source Data}

% After analyzing the previous part of the data, we found that in solving the competitive programs, using self\_contained, slib\_runnable, and plib\_runnable level data for finetune is the best. In this section, we analyze all self\_contained and slib\_runnable functions with docstring on GitHub, collecting a total of 1 million functions


% The file\_runnable level accounts for the largest proportion in open source projects, which is about 30\%. The second-highest percentage is the class\_runnable level, which accounts for 28\%. The slib\_runnable level accounts for only 6\%. 
% In addition, we can find that the first three types (i.e., self\_contained, slib\_runnable, and plib\_runnable) account for only 26\%. That is, the existing benchmark can only test about 26\% of the data in open source projects. 
% This ratio is far from sufficient. Therefore, the benchmark (\wenwangbench{}) for realistic development scenarios is provided later in this paper to alleviate this issue.

==> approach/model.tex <==
\subsection{Model: \wenwangcoder{}}
\label{sec: wenwang}


In this section, we introduce \wenwangcoder{}, a model fine-tuned on \codePLM{} using the \wenwangdataset{} with a \technique{} fine-tuning technique to improve the code generation capability of a pre-trained model on generating the code beyond standalone functions.
The reason why we chose PanGu-Coder as the finetuning model is that among the open-source models with a model size of 300M, PanGu-Coder performs best on HumanEval.
%The key idea is to fine-tune the pre-trained model with contextual information, to enhance its awareness of the context when generating code in practice.

The motivation behind our \technique{} fine-tuning technique lies in the observation of the function in the 100 most popular open-
source projects: more than 70\% are non-standalone functions, indicating that most functions in practice invoke or access non-built-in functions and non-standalone libraries.
From the view of code generation models, to generate non-standalone functions correctly, the docstring (natural language description) is not enough as the prompt for the model. Instead, contextual information is necessary and critical.
The model should be aware of the contextual information when inferencing, which requires it to be trained with such information as input.
However, since the previous models (i.e., Codex-S and PanGu-FT) are fine-tuned on only standalone functions to optimize the performance on HumanEval, they still lack the ability to make use of the context around the code to generate.
This gap motivates us to improve the existing pre-trained models through the fine-tuning stage.

We propose a \technique{} fine-tuning technique that aims to resolve the following two questions: what to use as the context and how to combine it with the original prompt (i.e., the docstring).

For the first question, since the \wenwangdataset{} includes the enclosing file content for each function, we are able to use either the raw contextual code text (similar to what Copilot does) or the program analysis results as the contextual information~\cite{CHENG2022contextual1, kanade2020contextual2,wang2021contextual3}.
We experiment with both options and conclude that the first one was rather limited and unstable, especially for longer files and models with small window sizes (say 1024 for \codePLM).
Therefore, we adapt the second option and extract the contextual information in a simple but intuitive way, that is, parsing the file content into an AST and extracting the label of all import statements and definition nodes, and concatenating these labels according to the contextual information of the function. 
This way of selecting contextual information can not only shorten the input of contextual information, but also contain as much important contextual information as possible.
For example, for a function that contains tokens in the class, the imported library names and the class member signatures are concatenated as the context, as shown in Figure~\ref{fig.prompt}.
Additionally, we also divide the contextual information into two types: all\_context (all the contextual information in the current file) and oracle\_context (the actually-used contextual information in the ground truth solution), to study whether the model can learn to select the useful context correctly.

\begin{figure}
	\centering
	\includegraphics[width=1.0\linewidth]{figure/Prompt_Construction.pdf}
	\caption{An Example of Prompt with Context}
	\label{fig.prompt}
\end{figure}


For the second question, we experiment with five ways of combining the context with the original docstring to construct a new prompt for the model and adapt the best one to produce \wenwangcoder{}.
Specifically, the combinations include: \textit{all\_context + docstring}, \textit{docstring + all\_context}, \textit{docstring + all\_context + docstring}, \textit{oracle\_context + docstring}, and \textit{docstring + oracle\_context}.
\textit{Oracle\_context} information refers to the information that the original function body actually depends on.
\textit{All\_context} information refers to all types, variables, and APIs defined/imported in the current file.
We use the \textit{only\_docstring} as the baseline for comparison and process \wenwangdataset{} to five different versions, each of which replaces the original prompt with these new prompts.
The main purpose of using \textit{oracle\_context+docstring} and \textit{docstring+oracle\_context} is to observe the performance of the model when providing the actual tokens that will be called in the generated code to the model. Due to the inability to know in advance the actual token called in the generated code before generating the code, we provide all\_context information. For all\_context information, we choose three combinations: \textit{all\_context+docstring}, \textit{docstring+all\_context}, and \textit{docstring+all\_context+docstring}. The reason for these combinations is to investigate how the order of all context information and docstring will perform on the model finetune. The experimental results show that \textit{all\_context+docstring} has the best effect. After analyzing the reasons, we believe that the combination of docstring in the final stage is consistent with pre-training, thus achieving the best effect.
Next, with the same hyper-parameters, we fine-tune \codePLM{} on these datasets independently to get 5 fine-tuned models and test their performance with the corresponding prompt format on \wenwangbench.
The result shows that any combination of the contextual information and the docstring could improve the performance comparing \textit{only\_docstring}, while \textit{all\_context + docstring} brought the most significant improvements.
We find that even prompting with other combinations, the model fine-tuned with \emph{all\_context+docs} still performs best and even better than the model specifically fine-tuned on that combination.
Therefore, we finally produce \wenwangcoder{} in this way.
Table~\ref{tab: The performance of wenwangcoder finetuned on different prompt and on different input prompts} shows the performance of different models fine-tuned on \codePLM{} by various context and docstring combinations.

The performance of the model fine-tuned with \textit{only\_docstring} (short as WWDocs) is lower than that of PanGu-Coder, while the performance of other models (except \textit{docstring + all\_context} in Pass@1) is always better than that of PanGu-Coder. This performance illustrates the importance of contextual information in generating code beyond standalone functions.
\begin{table}[th]
    \centering
    \footnotesize	
    \setlength\tabcolsep{1pt}
    \caption{Performance of models fine-tuned by various context and docstring combinations}
    % \vspace*{-1.5ex}
    \label{tab: The performance of wenwangcoder finetuned on different prompt and on different input prompts}
    \begin{tabular}{@{}llrrr@{}} 
        \midrule
        Fine-tune Prompt Type & Inference Prompt Type & pass@1 & pass@5 & pass@10\\
        \midrule
        AllContext+Docs & AllContext+Docs & \textbf{16.04\%} & \textbf{25.43\%} & \textbf{30.00\%} \\
        \midrule
        Only Docs & Only Docs &  15.3\% & 22.71\% & 26.09\% \\
        \midrule
        Docs+AllContext & Docs+AllContext & 15.7\% & 24.33\% & 29.57\% \\
        \midrule
        Docs+AllContext+Docs & Docs+AllContext+Docs & 15.78\% & 24.71\% & 29.13\% \\
        \midrule
        OracleContext+Docs & OracleContext+Docs & 17.04\% & 24.76\% & 28.26\% \\
        \midrule
        Docs+OracleContext & Docs+OracleContext & 16.43\% & 23.7\% & 27.39\% \\
        \bottomrule
    \end{tabular}
    \vspace*{-2.5ex}
\end{table} 
% Due to the page limitation, we leave the detailed experiment results of models fine-tuned by various context and docstring combinations in the supplementary appendix.  
%值得注意的是，Only Docs模型的效果要低于PanGu-Coder，而其他模型的效果（除了Docs+AllContext的Pass@1）几乎都优于PanGu-Coder。这充分说明了在生成non-standalone函数时，提供上下文信息的重要性。

% Although we only fine-tuned \codePLM{} with our dataset and approach for experimentation, the idea can be applied to any pre-trained models to optimize their performance on the pragmatic generation of code.


==> coverletter.tex <==
Cover Letter
Dear EIC, AE, and reviewers,
Thank you very much for considering our submission in the reviewing process!
This submission entitled “DeCon: Detecting Incorrect Assertions via Postconditions
Generated by a Large Language Model” presents our research efforts
on detecting incorrect assertions generated by a large language model.
We believe that the content of this submission is important to the computing field and
could gain the general interest of the journal readers for the following main reasons. 

We conduct an empirical study on the quality of assertions generated by four LLMs on
HumanEval and find that 62.4\% of generated assertions are incorrect.
• We propose a new approach named DeCon for detecting incorrect assertions by generating postconditions.
• DeCon not only detects an average of more than 64\% (63\% and 65.5\% detected by GPT-3.5 and
GPT-4, respectively) incorrect assertions generated by four LLMs but also further improves
the effectiveness of an LLM in the tasks of code generation and fault finding. 
Thanks for your great efforts on reviewing and considering this submission!
Best regards,
Hao, Tianyu, Jiaming, Zongyang, Yibo, Ying, Xinyu, and Tao.


==> dataavailability.tex <==
\section{Data Availability}
We have released all of the evaluation results on our anonymous website~\cite{sourcedata}.
We plan to publicly release our dataset at the publication time of our paper. 
At the current time of submission, we do not release our code repository as constrained by the public-disclosure requirement imposed  by our industrial collaborators at the moment; it would take some time to lift this requirement.


==> dataset.tex <==
\section{Dataset}~\label{sec: dataset}
In this section, we propose \javadata{}, an advanced dataset consisting of Java vulnerability description and their affected libraries.
As illustrated in Figure~\ref{fig : dataset}, we construct \javadata{} with three steps: 
(1) We collect the description of Java vulnerabilities and libraries;
(2) We collect the mapping between vulnerabilities and their affected libraries as positive samples;
(3) We collect the description of vulnerabilities of other programming languages to construct negative samples;
(4) We conduct data cleaning over the description in both positive samples and negative samples.

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{figures/dataset.pdf}
\caption{High level framework of \javadata{}{}}
\label{fig : dataset}
\end{figure}


\subsection{Data Collection}
\subsubsection{Description Collection} 
As mentioned in Section~\ref{sec:approach}, we take the description of vulnerabilities and libraries as the input of our model, the first step of dataset collection is to collect these descriptions.
For vulnerability description, we choose NVD~\cite{nvd} as the description resource. 
We collect all the vulnerability descriptions until 2022.03.31 from NVD.
Here, the latest CVE of vulnerabilities is CVE-2022-27216.
As for library description, we choose CPE~\cite{cpe} as the description resource.
In CPE, we collect 435,642 maven libraries and 310,844 of them have descriptions.

\subsubsection{Positive samples}
Besides collecting the descriptions, the most important step is to label the affected libraries of vulnerabilities.
Here, we denote the positive samples as the labels of real Java vulnerabilities and the labels of other vulnerabilities as negative samples.
The data we use to construct positive samples comes from two resources: GitHub Adversory~\cite{githubAD} and the vulnerability database manually labeled by our senior engineers.
We collect the labels of 583 Java vulnerabilities from GitHub Advisory and the labels of 2,206 ones from our vulnerability database.
Additionally, the labels of these 2,789 vulnerabilities have been manually checked with double-blind.




\subsubsection{Negative samples}~\label{sec: negative samples}
After collecting vulnerability entries, we add negative samples, which consist of vulnerabilities of programming languages besides Java, such as C/C++, and Python, into \javadata{} for two major reasons.
First, negative samples can improve the generalization ability of identification approaches. 
For a given vulnerability of other programming languages, an ideal identification mode should output no affected libraries. 
Thus, these negative vulnerability samples can help our model to learn their features.
Second, we cannot directly filter these negative samples because the programming language of vulnerabilities is not listed in modern vulnerability databases, such as NVD. 
Additionally, negative vulnerability samples count for a large portion of vulnerabilities.
According to our manual labeling, Java vulnerabilities count for about 2.5\% of all vulnerabilities.
Therefore, when applying an identification approach to a new vulnerability, it is likely to face vulnerabilities of other programming languages, thus requiring this identification approach to identify negative samples.

\subsection{Data Cleaning}
Before using collected data for model training, we conduct data cleaning on them with the following four steps:
\begin{itemize}
    \item We expand the apostrophes in the description. Listing~\ref{lst: apostrophes} shows the Python code of this procedure.
    \item We change the capital letters to lower letters.
    \item We replace all non-alphanumeric characters with spaces to split the description. 
    \item We remove the stopwords~\cite{ghag2015comparative}, which are frequently occurring words that hardly carry any information and orientation, such as ``the'', ``is'', ``have''. They are commonly removed in natural language processing tasks~\cite{ghag2015comparative, kaur2018systematic}.
\end{itemize}


\begin{lstlisting}[language = python, caption = Apostrophe expanding, label = lst: apostrophes]
def expand_apostrophe(inputString):
    text = re.compile("(it|he|she|that|this|there|here)(\'s)", re.I)
    text = pat_is.sub(r"\1 is", inputString)
    text = re.sub(r"won't", "will not", text)
    text = re.sub("(?<=[a-zA-Z])\'s", "", text)
    text = re.sub("(?<=s)\'s?", "", text)
    text = re.sub("(?<=[a-zA-Z])\'t", " not", text)
    text = re.sub("(?<=[a-zA-Z])\'d", " would", text)
    text = re.sub("(?<=[a-zA-Z])\'ll", " will", text)
    text = re.sub("(?<=[I|i])\'m", " am", text)
    text = re.sub("(?<=[a-zA-Z])\'re", " are", text)
    text = re.sub("(?<=[a-zA-Z])\'ve", " have", text)
    text = text.replace('\'', ' ')
    return text
\end{lstlisting}

% Before training the models, we preprocess the data in several steps. 1. Data Cleaning. We check the vulnerability reports in the dataset to ensure that their information is correct and up-to-date. For this purpose, we utilize the API provided by NVD\footnote{https://nvd.nist.gov/vuln/data-feeds} and compare the information retrieved from the API with the dataset. From the
% Figure 3: Distribution of the number of labels that the entries are related to
% 7,696 vulnerability reports that we checked, we find that 30 of them are no longer in use (e.g., no longer deemed a vulnerability, rejected by NVD, etc.). After removing these entries, our dataset has 7,666 vulnerability reports.
% 2. Label Merging. Next, we check the labels of the remaining 7,666 vulnerability reports and find that there are labels that always co-occur, which is a known problem in XML tasks [32, 51]. We find that the majority of co-occurrences are between labels that are closely related, such as gnome-session and gnome-shell. Therefore, we merge the labels that always co-occur into a single label. For example, the labels gnome-session and gnome-shell are merged into gnome-session;gnome-shell. We merged a total of 1,865 labels, reduc- ing the number of labels from 4,682 to 2,817. Figure 3 shows the distribution of the number of labels per vulnerability.
% 3. Feature Engineering. From each vulnerability report, we use its vulnerability description, references, and CPE configurations for training the models. We perform the same preprocessing steps as prior work [11]. While all three components are textual, we preprocess the components differently:
% • Description:Fromthedescriptiontext,weremovenon-alphanumeric characters and non-noun words. Non-alphanumeric char- acters are removed using a regular expression. Meanwhile,
% we remove the non-noun words using the part-of-speech tagging provided by NLTK [6] library. Following Chen et
% al. [11] work, we also remove words that appear in more than 30\% of the vulnerability data (i.e., common words). To do so, we use CountVectorizer from Scikit-Learn [36] to count the occurrences of each word in the vulnerability data.
% • References: We remove the non-alphanumeric characters from references. As an example, consider the reference link “http://secunia.com/advisories/59328” from CVE-2014-1533. We replace non-alphanumeric characters with whitespace,
% resulting in the following string: http secunia com
% advisories 59328.
% • CPE configurations: For each CPE configuration, we use a
% regular expression based on the CPE format [7] to retrieve the library names in the CPE. Consider the following CPE configuration for CVE-2014-1533: cpe:2.3:a:mozilla: firefox:*:*:*:*:*:*. Using the regular expression, we retrieve the library name mozilla firefox.
% After preprocessing, we concatenate the text into a single docu- ment. Then, the features for the XML models are extracted.
% 4. Train and Test Data Preparation. For a fair comparison between the models, we use the same training and testing dataset. Similar to Chen et al. [11], we use a 75\%-25\% split, where 75\% of the dataset forms the training dataset while the remaining 25\% forms the test dataset. This evaluation strategy is the standard approach in the literature of XML [3, 23, 26, 29, 39, 40, 52]. As each instance in the dataset may have multiple labels, we use iterative stratification [42, 45] to split the dataset, which is recommended for experiments on multi-label datasets [10, 43]. We use scikit- multilearn’s implementation2 to split the dataset. This results in a split where the training dataset has 6,017 entries and the test dataset has 1,649 entries.




% The data we use as our model inputs consists of two parts: the vulnerability description and the library description.
% We obtain vulnerability description from NVD and library description from CPE. 

% 394 bility database for constructing the training dataset, which maps
% 395 NVD data to the library names

% 435,642 -> 310,844

% until 2022.03.31
% 583 from github


==> evaluation/rq1_back.tex <==
% \subsection{RQ1: How do CodeGen, \codePLM{}, and \wenwangcoder{} perform on HumanEval and \wenwangbench{}?}
\subsection{RQ1: How do \wenwangcoder{}, PanGu-FT, and other two pre-trained models perform on HumanEval and \wenwangbench{}?}
% In this section, we first show the overall performance of \codePLM{}, CodeGen, and \wenwangcoder{} on HumanEval and \wenwangbench{}.
% Then we show the complementarity of the number of correct generating functions between the 3 models.
% Finally, we detail the different performance of the 3 models with multi-variants combination of contextual information.

\subsubsection{Overall performance}
\label{sec.rq1}

Table~\ref{tab: overall performance for wenwangbench and he} shows the overall performance of CodeGen, \codePLM{}, and \wenwangcoder{} on HumanEval and \wenwangbench{}. 
\wenwangcoder{} consistently outperforms CodeGen and \codePLM{} at all Pass@Ks on both \wenwangbench{} and HumanEval.~\footnote{HumanEval scores are slightly different from the CodeGen and \codePLM{} paper because they used \emph{n}=200 in experiments.}
On \wenwangbench{}, \wenwangcoder{} outperforms CodeGen by 5.22\% when generating only one solution and by 5.17\% when recommending one from 10 generated solutions.
Comparing with its baseline model \codePLM{}, \wenwangcoder{} brings an improvement of 3.05\% on Pass@1 (greedy), and 2.47\%, 2.56\%, 1.74\% when generating 10 solutions.
Although \wenwangcoder{} is designed to enhance the capability to generate non-standalone functions, the standalone function generation ability inherited from \codePLM{} does not degrade on HumanEval.

% From the table, we can also observe that on \wenwangbench{}, CodeGen is less effective than \codePLM{} at Pass@1, but outperforms \codePLM{} at Pass@5 and Pass@10. 
% In addition, the gap between CodeGen at Pass@5 and Pass@10 metrics is narrowed compared to Wenwang at Pass@1 performance.
% This shows that CodeGen is more capable of generating diverse code than \codePLM{}.

\begin{table}[t]
    \centering
    \footnotesize
    \setlength\tabcolsep{1.4pt}
    \caption{RQ1: Main Results for 3 Models on 2 Benchmarks}
    % Pass@K for \codePLM{}, CodeGen, and \wenwangcoder{} on \wenwangbench{} and HumanEval}
    \vspace*{-1.5ex}
    \label{tab: overall performance for wenwangbench and he}
    \begin{tabular}{@{} ccc|ccccc @{}} 
        \toprule
        \multicolumn{1}{c}{\multirow{2.5}{*}{Benchmark}} & \multicolumn{1}{c}{\multirow{2.5}{*}{Model}}
        & \multicolumn{1}{c|}{n=1} & \multicolumn{3}{c}{n=10}\\
         \cmidrule(lr){3-6}
        & &  Pass@1(greedy) & Pass@1 & Pass@5 & Pass@10\\
        \midrule
        \multirow{3}{*}{\wenwangbench{}} & CodeGen &    10.87\%    & 9.26\% & 21.29\% & 25.22\% \\
        & \codePLM{} &  13.04\%  &   11.96\% & 19.73\% & 23.91\% \\
        & PanGu-FT &  -\%  &   13.09\% & 19.80\% & 22.61\% \\
        & \wenwangcoder{} & \textbf{16.09\%}  & \textbf{14.43\%} & \textbf{22.29\%} & \textbf{25.65\%} \\
        \midrule
        \multirow{3}{*}{HumanEval} & CodeGen &   10.98\%     & 9.76\% & 18.85\% & 22.56\% \\
        & \codePLM{} &   17.07\%    & 13.23\% &20.46\% & 22.56\% \\
        & PanGu-FT &  -\%  &   19.50\% & -\% & 25.96\% \\
        & \wenwangcoder{} &  \textbf{17.68\%}  & \textbf{15.92\%} & \textbf{21.76\%} & \textbf{23.17\%} \\
        \bottomrule
    \end{tabular}
    \vspace*{-2.5ex}
\end{table} 


\subsubsection{Detailed Comparison}

Figure~\ref{fig.complenment_overall} shows the number of solved problems by the three models on \wenwangbench{}, with the difference and overlapping.
We consider a problem to be solved if the model can generate \emph{at least} one correct solution that passes all tests out of the ten generated solutions.
Among the 230 problems in \wenwangbench{}, the total number of problems solved by the three models is 88 (union), while 48 problems can be solved by any of the three models (intersection).
Compared with \codePLM{}, \wenwangcoder{} additionally solves 11 different problems, while failing to solve four that \codePLM{} should have solved. We dive into the concrete cases and find that three of them rely on standard or public libraries (one slib\_runnable and two plib\_runnable). For these problems, although \wenwangcoder{} is prompted with the imported libraries in the current file, it fails to use the correct library or API to fulfill the correct implementation.


\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{figure/complementarity-overall.pdf}
	\caption{Number of correctly-generated functions of CodeGen, \codePLM{}, and \wenwangcoder{} on \wenwangbench{}}
	\label{fig.complenment_overall}
 \vspace*{-2.5ex}
\end{figure}

 


Table~\ref{tab: mult performance on wenwangbench} shows the performance of three models on the six types of functions in \wenwangbench{}.
The type of function represents the non-overlapping part between two neighboring runnable levels in Figure~\ref{fig.run_dep_res}. For example, the class\_depended represents those functions that must depend on other code in the current class.
While \wenwangcoder{} outperforms CodeGen and \codePLM{} at self\_contained, class\_depended, and file\_depended levels, it slightly downgrades at slib\_depended, plib\_depended, and project\_depended levels, which is consistent with the above case study on the 4 cases that \codePLM{} succeeds but \wenwangcoder{} fails.
By comparing the generated code manually, we find that \wenwangcoder{} is more capable of understanding and using the provided context to generate code compared with the other models.
Particularly, at the class\_depended and file\_depended level, where the function is expected to use the existing code in the current class or file, \wenwangcoder{} is better at selecting and using the correct functions and variables, so it obviously outperforms \codePLM{} by a large margin.
However, at the slib\_depended and plib\_depended level where the function is expected to use the API provided by libraries, \wenwangcoder{} seems to be overwhelmed by the contextual information that tells it all the imported library names.
As there are many libraries and APIs in each library to choose from, it is difficult for the model to make the correct choice, although it seems simple and straightforward for experienced developers.
Based on this observation, we anticipate that it is a promising research direction to integrate API recommendation tools~\cite{Rahman2016APIreco1, huang2018APIreco2, li2018APIreco3} to recommend a set of possibly-used libraries/APIs as the context, which will significantly reduce the decoding space of large language models when in pragmatic code generation.


\begin{table}[t]
    \centering
    \footnotesize	
    \caption{Performance of 3 Models Across 6 Types of functions}
    \vspace*{-1.5ex}
    \label{tab: mult performance on wenwangbench}
    \begin{tabular}{@{}rcrrrrrrrr@{}} 
        \midrule
        Runnable Level &  \multicolumn{1}{c}{Model}  & Pass@1 & Pass@5 & Pass@10\\
        \midrule
        \multirow{3}{*}{self\_contained} &  CodeGen  &  17.14\% & 34.82\% & 37.14\% \\
        & \codePLM{} & 21.14\% &34.92\% & 40.00\% \\
        & \wenwangcoder{} & \textbf{28.00\%} & \textbf{39.85\%} & \textbf{42.86\%} \\
        \midrule
        \multirow{3}{*}{slib\_depended} &  CodeGen  & 8.21\% & 20.04\% & 25.00\% \\
        & \codePLM{} &  \textbf{12.50\%} & \textbf{24.89\%} & \textbf{32.14\%} \\
        & \wenwangcoder{} & 12.14\% & 20.55\% & 25.00\% \\
        \midrule
        \multirow{3}{*}{plib\_depended} & CodeGen & 9.52\% & 25.57\% & \textbf{33.33\%} \\
        & \codePLM{} & \textbf{16.67\%} & \textbf{27.49\%} & \textbf{33.33\%} \\
        & \wenwangcoder{} & 14.76\% & 21.32\% & 23.81\% \\
        \midrule
        \multirow{3}{*}{class\_depended} & CodeGen & 9.82\% & 24.24\% & 29.09\% \\
        & \codePLM{} & 10.55\% & 17.98\% & 23.64\% \\
        & \wenwangcoder{} & \textbf{17.45\%} & \textbf{27.02\%} & \textbf{30.91\%} \\
        \midrule
        \multirow{3}{*}{file\_depended} & CodeGen &  7.50\% & \textbf{16.15\%} & \textbf{19.12\%} \\
                & \codePLM{} & 9.85\% & 12.91\% & 14.71\% \\
        & \wenwangcoder{} & \textbf{10.15\%} & 15.90\% & \textbf{19.12\%} \\
        \midrule
        \multirow{3}{*}{project\_depended} & CodeGen & 2.17\% & 6.42\% & \textbf{8.70\%} \\
        & \codePLM{} & \textbf{2.61\%} & \textbf{7.63\%} & \textbf{8.70\%} \\
        & \wenwangcoder{} & 1.74\% & 6.16\% &  \textbf{8.70\%} \\
        \bottomrule
    \end{tabular}
    \vspace*{-2.5ex}
\end{table}

It is worth noting that all models perform very poorly at the project\_runnable level, which is not surprising considering the commonly-adopted self-supervised and auto-regressive pre-training method.
Currently, almost all these large generative models of code follow the architecture and training approach in natural language processing. They consider the source code as plain text and pre-trained a causal language model with the next-token-prediction within a source file. However, considering the cross-file context information in the prompt is necessary for pragmatic code generation in real projects, as a recent exploration study~\cite{repo_level} shows. We consider it to be our future work on a more \emph{intelligent} context-aware code generation.

% After the functions and variables related to the class and the current file are added in the finetune phase and code generation phase, \wenwangcoder{} can select the correct functions and variables in the current class and file to invoke, thereby improving the accuracy of code generation in the class\_runnable, and file\_runnable levels.

% After analyzing reasons, we think that it is not enough to introduce only the context information of the standard library and the public library, because each library may call many functions and variables, so it is difficult for the large language models to make a correct choice. 
% It would be an interesting research direction to recommend the functions and variables that may be called in the library based on the program context information and natural language description.

% Note that \codePLM{} outperforms CodeGen and \wenwangcoder{} on project\_level.
% This is not common sense, because for all models, finetune is only done at the file level, and pangu does not make sense to be more effective at the project\_runnable level than the CodeGen and \wenwangcoder{}. 
% According to the example analysis, all models generate incorrect answers at the project\_runnable level. 
% The reason why our verification platform judge these answers as correct is the return value of the test cases corresponding to these answers is None. 
% Therefore, the generated code is considered correct as long as no error is reported and no return value is returned during running.

% In Section~\ref{sec:discussion}, we will describe in detail the ratio of functions that do not return values to \wenwangbench{} and the experimental results after these functions are removed. 
% We find that the proportion of these functions is small, and our conclusions remain unchanged after removing these functions.

==> evaluation/rq3_back.tex <==
\subsection{RQ3: How does the performance of four models correctly utilise the contextual information? }

\begin{table}[t]
    \centering
    \footnotesize
    \setlength\tabcolsep{2pt}
    \caption{RQ3: The accuracy of three models that they can correctly generate the contextual tokens}
    \vskip 0.15in
    \label{tab: contextual}
    \begin{tabular}{@{} cc|cccccccc @{}} % suppress vertical whitespace at start and end
        \toprule
        % \multicolumn{1}{c}{\multirow{2.5}{*}{Model}} & \multicolumn{1}{c}{\multirow{2.5}{*}{Prompt}} 
        % & & \multicolumn{4}{c}{Python} & \multicolumn{4}{c}{Java} &
        \multicolumn{1}{c}{\multirow{2.5}{*}{Model}} & \multicolumn{1}{c}{\multirow{2.5}{*}{Contextual Type}}  & \multicolumn{4}{c}{Acc@K}\\
        \cmidrule(lr){3-6} 
        % & & \multicolumn{1}{c|}{n=1} & \multicolumn{3}{c}{n=10}& \multicolumn{1}{c|}{n=1} & \multicolumn{3}{c}{n=10}\\
        %  \cmidrule(lr){4-6}  \cmidrule(lr){8-10}
         & & Average& Acc@1 & Acc@5 & Acc@10\\
        \midrule
        \multirow{3}{*}{CodeGen} &  TypeReference  &  12.63\%&  13.01\% &  22.97\% & 25.93\% \\
        & APIInvocation   &  7.78\%&  7.04\%& 17.40\% & 21.90\%\\
        & VarReference   & 3.37\% & 3.45\% & 7.10\% &8.36\%\\
        \midrule
        \multirow{3}{*}{\codePLM} &  TypeReference  & 13.16\%&11.06\%&  22.80\% & 26.46\% \\
        & APIInvocation   & 6.64\%&5.95\%& 11.22\% & 14.53\% \\
        & VarReference  &3.15\%& 3.08\%& 4.60\% & 5.30\% \\
        \midrule
        \multirow{3}{*}{\wenwangcoder{}} &  TypeReference   & 19.98\%&21.54\%&  31.01\% & 34.48\% \\
        & APIInvocation   & 12.51\%&10.99\%&23.71\% &29.76\%\\
        & VarReference   & 4.12\%&4.20\%& 8.86\% & 11.04\%\\
        \bottomrule
    \end{tabular}
    \vspace*{-2.5ex}
    
\end{table} 

To further study the \emph{context-awareness} of large language models, we analyze the identifier tokens in generated code and focus on three types of tokens: TypeReference, APIInvocation, and VarReference (including constants reference).
Table~\ref{tab: contextual} shows the Acc@k of three models, we find it is consistent with Pass@K (i.e., the generated functions can pass test cases), and the Acc@K of Codex is also the best one in generating contextual dependency. 
To further explore the ability of different models in generating different types of context information, we divide the context token into three categories: TypeReference, APIInvocation, and VarReference, which usually form the most important part of the implementation at runnable-levels with external dependency.
%We do not classify constants because, in common programming habits, developers often use a global variable declaration for a constant, which is context-dependent. 
As shown in Table~\ref{tab: contextual}, on \wenwangbench{}, all models show poor effectiveness in generating the correct ``VarReference'' token, while the effectiveness in generating ``TypeReference'' token is relatively good.

Compared with \codePLM{} and CodeGen, \wenwangcoder{} performance best in correctly utilizing the contextual information.


% Table~\ref{tab: overall performance for wenwangbench} shows the overall performance of \codePLM{}, CodeGen, and \wenwangcoder{} on \wenwangbench{}. 
% As shown in the table, we find that when n is 10, whether k is 1, 5, or 10, \wenwangcoder{} is significantly better than \codePLM{} and CodeGen. Especially when k is 1, the effect of \wenwangcoder{} is much higher than that of \codePLM{} and CodeGen.


% Figure~\ref{fig.complenment_humanlabel} shows the number of functions that are correctly generated when replacing the original docstring with the human-labeled version.
% Overall, for all three models, the number of problems that are solved by only changing the docstring is 11, but interestingly, their intersection is only 1.
% This indicates different models' sensitivity to the prompt, as well as the complementarity in their capability.


% Figure~\ref{fig.case_humanlabel} shows an example function in \wenwangbench{}, with the two versions of docstrings and two solutions generated by \wenwangcoder{}.
% The task is to remove and return the first enqueued element from the data object.
% The left part shows the original docstring and an incorrect solution, which is incorrect because the generated code returns the last element instead of the first and does not remove it before returning.
% The right part shows the human-labeled docstring that details the expected behavior of the function and a correct solution that is different but equivalent to the original code.
% Due to the page limitation, we leave more examples in the supplementary appendix.
% \begin{figure}
% 	\centering
% 	\includegraphics[width=1.0\linewidth]{figure/HumanLabel_case_study.pdf}
% 	\caption{An example of the functions incorrectly generated with the original docstring but correctly generated with the human-labeled docstring}
% 	\label{fig.case_humanlabel}
%   \vspace*{-1ex}
% \end{figure}



% % We anticipate that the problem also exist in the pre-training dataset, The large language model is very sensitive to the prompt and more research work can be done in guiding the user to provide a proper docstring

==> introduction.tex <==
\section{introduction}
\label{sec.intro}

Recent years have seen a trend to apply machine learning techniques to open-domain code generation tasks, especially large language models~\cite{radford2018improving,brown2020language,gpt-neo,Mikel2019BART} based on Transformer~\cite{vaswani2017attention}, such as Codex~\cite{codex}, AlphaCode~\cite{alpha_code}, CodeGPT~\cite{lu2021codexg}, In-Coder~\cite{fried2022incoder},
CodeGen~\cite{nijkamp2022conversational}, \codePLM{}~\cite{fenia2022pangu}, StarCoder~\cite{li2023starcoder}, and WizardCoder~\cite{luo2023wizardcoder}.
These efforts typically involve pre-training on a large-scale corpus of code 
and further training (aka fine-tuning) using data of similar formats and distributions to the target downstream task, i.e., generating code from the given natural language description.
When pre-trained on a large-scale code corpus, a model widely learns the representation and distribution of source code written in various programming languages~\cite{liu2020pretrainadv1,lin2022pretrainadv2,guo2022pretrianadv3}.
When fine-tuned on relatively smaller datasets, the model concentrates on a specific domain or task input/output format to achieve better performance in the target downstream task~\cite{zhang2019finetuneadv1,sun2019finetuneadv2,li2021finetuneadv3}.
It is critical to prepare fine-tuning datasets of high quality and similarity to the target downstream task~\cite{liu2021datasetimport,codex,fenia2022pangu,korbak2022on}

Many existing large language models for code generation have the parameter size of billions, tens of billions, or even hundreds of billions. Although the effectiveness of code generation is getting better as the model's parameter size continues to increase, models that blindly pursue large-scale parameters waste a lot of computational resources and cause environmental pollution.
Existing works~\cite{codex,li2023starcoder} show that large language models with a parameter size of tens of billions emit a large amount of carbon dioxide, which not only wastes computing resources but also causes environmental pollution.

To alleviate the negative impact of blindly pursuing models that are too large, this paper focuses on how to improve the performance of models with a parameter size of 300 million in code generation tasks.
There are three main reasons why we chose a model with a parameter size of 300 million. First, the computing resources we have cannot support us to finetune a model of billions or even tens of billions. Second, from the perspective of environmental protection and energy conservation~\cite{rillig2023risks,bender2021dangers,hort2023exploratory}, models with larger parameter scales consume more resources during the stage of training and inference. Third, the larger the model parameter size, the slower the inference speed, and the worse the experience for developers when using it~\cite{wang2023tabi,jin2021good,park2022nuqmm}.

In the task of code generation, the target code being generated can be classified into two types: a \textit{standalone function} (i.e.,
a function that invokes or accesses only built-in functions and standard libraries) and a \textit{non-standalone function} (i.e., a function not being a standalone function). In open-source and proprietary code, there is a majority being non-standalone functions (e.g., more than 70\% among top 100 open-source projects based on stars in GitHub) ~\cite{yu2023ce}. 
For example, a typical function for calculating the value of the ``Fibonacci'' sequence belongs to a standalone function.
A function that  invokes or accesses non-built-in functions and non-standard libraries is a non-standalone function.
%Fetch the HEAD of the remote url to determine the content type.
%Dynamically create a Point subclass.


% However, existing fine-tuning datasets share a common limitation, as they include only standalone functions. 
% According to our statistics, 
% However, this kind of function accounts for less than 30\% in open-source projects~\cite{yu2023ce}, the existing datasets for fine-tuning mismatches the downstream task of generating code beyond standalone functions.
% In development scenarios, most functions rely on contextual information to fulfil their tasks~\cite{liu2018context1,Roehm2012context2,MAGUIRE2001context3}.
% Consequently, although the resulting models (fine-tune with datasets that contain only standalone functions) perform well for introductory competition problems and basic programming tasks (such as HumanEval~\cite{codex}), they do not pay attention to the fine-tuning process of generating the code beyond standalone functions.





To effectively generate functions of competitive programming (all being standalone functions), previous work~\cite{codex, fenia2022pangu} such as Codex~\cite{codex} and \codePLM{}~\cite{fenia2022pangu} typically collects fine-tuning datasets with only standalone functions. \textbf{Codex}. The authors of Codex collect 50,000 programming problems from two sources: 10,000 competition problems from competitive programming websites and 40,000 \textit{standalone functions} (i.e., a function that invokes or accesses only built-in functions and standard libraries) from open-source repositories.
In particular, among the code snippets from the two sources, the Codex authors select only those functions that (1) accept inputs and return outputs, (2) can be executed correctly and deterministically outside the enclosing project environment, (3) are not ambiguous or too difficult for the pre-trained Codex-12B~\cite{codex} model; the Codex authors determine a function to be ambiguous or too difficult when 100 samples (i.e., code snippets) generated with the pre-trained Codex-12B model for the problem derived from this function does not pass the unit tests associated with the function.
The authors of Codex produce Codex-S by fine-tuning Codex on the collected datasets. \textbf{\codePLM{}}. 
Similarly, the authors of \codePLM{} also collect data from both programming contests and open-source projects but do not filter the collected functions with a pre-trained model (as done by the Codex authors), resulting in 18,000 competition problems and 49,000 open-source functions.
The authors of \codePLM{} produce PanGu-FT by fine-tuning \codePLM{} on the collected datasets.
%Codex
Models (e.g., Codex-S, PanGu-FT) fine-tuned by existing fine-tuning datasets (containing only standalone functions) perform better than those without fine-tuning on HumanEval, which also contains only standalone functions.
Existing models can improve the performance of generating standalone functions from the model after using the dataset containing only standalone functions for fine-tuning.


To effectively generate code, especially for non-standalone functions (largely ignored by existing work),  
%instead of focusing on only standalone functions.
%To optimize pre-trained models for the task of generating code beyond standalone functions, 
in this paper, we propose \ww{}, a new approach to finetune a pre-trained model. 
As we observe that the target function's contextual information (i.e., code elements such as type reference, API, variable, and constant outside the function but within the dependent third-party libraries, current class, file, or project) is critical for generating a correct non-standalone function, the core idea of \ww{} is to improve a model's ability to be aware of and make use of the contextual information  through fine-tuning a model with a dataset that contains code beyond standalone functions and our \technique{} fine-tuning technique.
Compared to the models (e.g., Codex-S and PanGu-FT) with fine-tuning on only standalone functions, the functions included in the fine-tuning dataset used by \ww{} also include non-standalone functions. 
%Compared with the existing pre-training models (e.g., PanGu-Coder, CodeGen, and Codex), although these models can also capture contextual information within the scope of the sliding window, their performance to capture contextual information completely depends on the size of the sliding window. 
% When the size of sliding window for a model is limited, the performance of the model to capture contextual information is also limited.


In particular, \ww{} consists of two components: a fine-tuning dataset named \wenwangdataset{} that contains functions beyond standalone functions and a fine-tuned model named \wenwangcoder{} by fine-tuning a state-of-the-art model named \codePLM{}~\cite{fenia2022pangu}  with our \technique{} technique based on \wenwangdataset{}. \textbf{\wenwangdataset{}}. 
We start by constructing a dataset named \wenwangdataset{} for fine-tuning. \wenwangdataset{} consists of 103,541 Python functions with docstrings, code snippets, and other information.
All functions in \wenwangdataset{} are covered by tests.
A recent study~\cite{codex} shows that functions covered by tests are likely to be correct and well-written.
Unlike existing datasets~\cite{codex,fenia2022pangu}  that contain only a small subset of real-world functions, \wenwangdataset{} comprehensively covers most types of functions, regardless of the used data types and the depending code elements outside the target function.
% Then, we fine-tune a state-of-the-art model \codePLM{} on \wenwangdataset{} to produce a model named \wenwangcoder{} and conduct experiments to compare its performance with the other public available models: CodeGen, \codePLM{}, and PanGu-FT.
\textbf{\wenwangcoder{}}. Then, we fine-tune the \codePLM{} on \wenwangdataset{} with our \technique{} fine-tuning technique so that the contextual information can be fully leveraged during code generation.
The reason why we chose PanGu-Coder as the finetuning model is that among the open-source models with a model size of 300M, PanGu-Coder performs best on HumanEval.
% There are three main reasons why we chose a model with a parameter size of 300 million. The first reason is limited by computing resources. The computing resources we have cannot support us to finetune a model of 6 billion or even 10 billion. The second is that from the perspective of environmental protection and energy conservation, models with larger parameter scales consume more resources during inference. The third reason is inference speed. The larger the model parameter size, the slower the inference speed, and the worse the experience for developers when using it.
We design our \technique{} fine-tuning technique to address the following two questions: what to use as the context and how to combine it with the original prompt (i.e., the docstring).
For the first question, we parse the file content into an AST (Abstract Syntax Tree) and extract the label of all import statements and definition nodes, and concatenate these labels to produce the context.
For the second question, we experiment with five ways of combining the context with the original docstring to construct a new prompt for the model and adopt the best way.

To evaluate the performance of \wenwangcoder{}, we not only focus on the HumanEval benchmark but also pay more attention to CoderEval~\cite{yu2023ce}, a recent benchmark that can be used to assess the performance of the models to generate non-standalone functions. 
CoderEval contains both standalone functions and non-standalone functions.
Compared with HumanEval (all functions are standalone functions), CoderEval can be used to assess the performance of a model in generating code beyond standalone functions.
The experimental results show that through a fine-tuning process with a dataset that contains both standalone functions and non-standalone functions, and a \technique{} fine-tuning technique, \wenwangcoder{} outperforms PanGu-FT and the other two pre-trained models (i.e., CodeGen and \codePLM{}) both on \wenwangbench{} and HumanEval.


In summary, we make the following main contributions:
\begin{itemize}
    \item We propose Wenwang, an approach based on a pre-trained model to generate code beyond standalone functions, consisting of (1) a fine-tuning dataset named WenwangData that contains both standalone functions and non-standalone functions and (2) a fine-tuned model named WenwangCoder by fine-tuning PanGu-Coder with our context-aware technique based on WenwangData.

    \item We conduct experiments to show that WenwangCoder not only outperforms three models (i.e., CodeGen, PanGu-Coder, and PanGu-FT) on both CoderEval and HumanEval, but also outperforms ChatGPT in generating non-standalone functions on CoderEval (Pass@5 and Pass@10), demonstrating the benefits and performance of WenwangCoder. 
    \item We study the performance of different models that vary for different context types, formats, and prompts on CoderEval and highlight the importance of contextual information in both the training and inference stages for the task of code generation.


    %Experimental results show that \wenwangcoder{} outperforms PanGu-FT and the other two public available models both on \wenwangbench{} and HumanEval.
    
    % \item We trained a model named \wenwangcoder{} by fine-tuning \codePLM{} with a explicit context-aware technique based on \wenwangdataset{}.

    
    % \item We construct a high quality (i.e., covered by tests) and pragmatic dataset named \wenwangdataset{} for fine-tuning to reduce the gap between existing models with fine-tuning and the task of pragmatic code generation.
    
    % \item We trained a model named \wenwangcoder{} by fine-tuning \codePLM{} with a explicit context-aware technique based on \wenwangdataset{}.

    % \item We study the pragmatic aspect (e.g., different contextual information and different prompts) of fine-tuned/pre-trained code generation models and highlight the importance of contextual information in both the training and inference stages for the pragmatic generation of code.
\end{itemize}

The remainder of this paper is organized as follows. Section~\ref{sec:background} introduces the background and related work of code generation. Section~\ref{sec:approach} details  \ww{}, consisting of  \wenwangdataset{} and \wenwangcoder{}.  Sections~\ref{sec:evaluation} and ~\ref{sec:experiments} describe the experimental setup and experimental results. 
Section~\ref{sec:discussion} discusses our work.
Section~\ref{sec:conclusion} concludes this paper.

% ------------------BACKUP--------------------------

% Two limitations can be identified from previous datasets: 
% First, they are limited to introductory competition problems and basic programming tasks, thus are too simple to act as a proxy of practical use scenarios.
% Originally, Codex and \codePLM{} constructed the dataset to improve the models' performance on the HumanEval benchmark, which contains only 164 hand-written programming problems and corresponding unit test cases. Therefore, the fine-tuning dataset are constructed to only include functions that purely use basic data types and can run independently.
% Second, they only consider the function docstring as input, and the code snippet in function body as expected output, but does not consider the context of the function such as the used library, the class and file, and other reference context code in other files of the current project. However, in real development scenarios, most functions depend on these context information to fulfill their tasks~\cite{liu2018context1,Roehm2012context2,MAGUIRE2001context3}.
% Third, none of their finetuning datasets are open source.
% Neither Codex nor \codePLM{} disclosed their finetuning datasets, significantly hindering the following research works to replicate and further improve the approaches.
% As a result, it is difficult to use the fine-tuning dataset constructed by Codex and \codePLM{} optimize the performance of code generation models in the realistic development scenario.


% Similar to HumanEval, each sample includes the function's docstring, signature, code snippet, and multiple test cases, thus enabling automatic evaluation of the behavior correctness of generated code in term of the \textit{Pass@K} metric.
% Different from HumanEval, \wenwangbench{} (1) categorizes the data into different levels (from self-contained to project-runnable) according to the scope of context required to run the function, to simulate the distribution of normal functions in general open-source projects, (2) considers project-defined data types instead of basic data types in the Python language, and (3) additionally provides a human-labeled version of the original docstring, and allows for adding the contextual information to facilitate the generation.
% We provide a ready-to-use environment/platform to execute generated code snippets in the successfully-built projects, to simulate the code generation and verification process in realistic contexts.
% To verify the effectiveness of \wenwangdataset{}, we further \wenwangcoder{} exhibits better performance on both \wenwangbench{} and HumanEval compared with CodeGen and the baseline model \codePLM{}, showing that our dataset do have the potential to bring positive improvements to existing models in the pragmatic code generation task.


% solutions from several popular programming contest and
% interview preparation websites
% The performance of such models heavily relies on the underlying dataset, a high-quality dataset with the same distribution with the downstream tasks is important. To automatically evaluate the correctness of the code generated by large language models, a high quality benchmark is needed.
% Dataset and benchmark are all very important for large language model.


% For dataset, the SOTA model --- Codex by Microsoft and OpenAI, as the first model that has been put into mature product (GitHub Copilot), again proved the great influence of high-quality dataset on finetuning the model towards the target downstream task. [Write how Codex collect and use their dataset to achieve an improvement of 6-40 points on the HumanEval benchmark] the high-quality dataset used by Codex contains two parts: from competitive programming websites and from open source repositories with continuous integration. The first part collects data from competitive programming, resulting 10,000 problems. The second part collects data from open source projects, resulting 40,000 problems. The authors of codex named the Codex with supervised finetuning data as Codex-S. Codex-S can achieve an improvement of 6-40 points on the HumanEval benchmark.


% To address the preceding limitations, in this paper, we start by reproducing the finetune data of Codex and \codePLM{}, and additionally enhanced it to present and publish a high-quality, contextual-enhanced, muti-runnable, continuously-evolving, and community-driven dataset.
% For the construction of the high-quality dataset, we think that the quality of the code that is covered by the test case and passes the test case is high. 
% We reproduce the finetune data of Codex and \codePLM{}, we considered public Python repositories on GitHub using Travis or Tox as their continuous integration (CI) system(s). 
% We reproduced the CI environment of each project locally in docker instances, then injected a tracing function in the environment, which would capture the input, output, invocation location and context code for each function invoked during integration testing. 
% After that, the CI script was triggered and the data of invoked functions were recorded into a database. 
% To construct the muti-runnable dataset, we propose an algorithm of multiple runnable algorithm to construct the dataset. 
% To construct the continuously-evolving and community-driven dataset, we analyze the push time for each file and public a mongo database that allows developers to contribute. 
% We hope that both researchers and practitioner's can make use of it to finetune the existing pre-trained code models on concrete development tasks, to boost the application of models into developers' real daily work.


% After the pre-trained model is trained with the high-quality finetune dataset, the effect of the pre-trained model after finetune needs to be tested on the high-quality benchmark. 
% Currently, the most commonly used benchmark for verifying the effect of large models is HumanEval\footnote{\url{https://www.github.com/openai/humaneval}}. HumanEval is constructed by Codex, it contains 164 hand-written programming problems. Each problem includes a function signature, docstring, function body, and several unit tests. 
% The reason why codex construct the benchmark (i.e., HumanEval) with hand-written is Codex can make the data in benchmark not appear in the training set. 
% Although Codex can ensure the data the HumanEval benchmark not appear in the training set, it only uses to validate the corrections of competitive problems. Thus the HumanEval benchmark is limited in validating the code in real development scenarios.

% To address the preceding limitation, we construct a real-development-use-oriented benchmark for the natural language code generation task, multiple runnable level, method signature, docstring, test cases, and the ground truth code. 
% We denote the benchmark as \wenwangbench{}.
% To ensure the data in \wenwangbench{} is not appeared in the training set, we only collect the data (with docstring, test cases) submitted after 1, January, 2022 from GitHub\footnote{\url{https://www.github.com}}. In totally, \wenwangbench{} contains 210 functions.
% To make \wenwangbench{} can validate the code with multiple runnable level, we classify the data in \wenwangbench{} into six runnable level: self\_contained, slib\_runnable, plib\_runnable, class\_runnable, file\_runnable, and others. We build an automated evaluation platform to evaluate the correctness of the code produced by large language model automatically. 
% To ensure the quality of the docstring of these code snippet, besides the original docstring in the open source projects, we also add the docstring rewrote by developers, which can make the docstring in \wenwangbench{} more reliable.

% In this paper, we first construct a finetune dataset named \wenwangdataset{} for the task of pragmatic code generation.
% Then we use \wenwangdataset{} to finetune \codePLM{} to produce \wenwangcoder{}.
% Finally, we construct a real-development-use-oriented benchmark and validation platform named \wenwangbench{}.
% Experiment results show that \wenwangcoder{} can not only perform well on HumanEval benchmark than \codePLM{} and CodeGen, but also perform well on \wenwangbench{} than \codePLM{} and CodeGen.
% Our work can help researchers to 
% understand the advantage and limitation of each model in fine-grained scenarios, to shed light on the future research direction in this field.

% In this paper, we start by reproducing the supervised finetuning data of Codex-S, and additionally enhanced it to present and publish a high-quality, continuously-evolving, community-driven dataset.
% We hope that both researchers and practioners can make use of it to finetune the existing pretrained code models on concrete development tasks, to boost the application of models into developers' real daily work. We also discuss the next step of code generation from a more software engineering viewpoint.




%  Some prompts
% underspecify the function that is implemented, in which
% case a perfectly valid solution may be wrongly penalized by
% the unit test

==> related_work.tex <==
\section{Related Work}\label{sec:related}
In this section, we introduce related works.
We first introduce related works about unit test generation.
Then we introduce related works about unit test parameterization. 
\subsection{Unit test generation}
In recent years, with the wide adoption  of object-oriented programming~\cite{oop1,oop2}, object-oriented unit testing~\cite{oopt1,oopt2,oopt3} has received high attention. 
Object-oriented unit test generation tools not only need to generate input parameters, but also need to generate test sequences. 
Evosuite recursively creates test sequences that satisfy all dependencies by considering the return types of all methods. 
Evosuite uses centralized local search and dynamic symbolic execution after each predefined number.  
Randoop incrementally creates test sequences, and sequences that exhibit illegal behavior are discarded. Only sequences with normal behavior are used to generate new sequences, because extending a sequence that contains a corrupted state makes little sense.  
Randoop predefines some fixed values for each input parameter with primitive type, string type, and some values defined in the code context.
EvoObj~\cite{evoobj} is implemented on the top of Evosuite, it constructs an object construction graph for a function under test to synthesize test template code to result valid objects. 

\subsection{Unit test parameterization}
Tillmann et al.~\cite{tillmann2005parameterized} present the concept of parameterized unit tests, and showsummarize three different methods' behavior: state change, normal return value, and exceptional return.
They also demonstrate the ability of parameterized unit tests to find bugs in the .net framework library.
Thummalapenta et al.~\cite{put4} conduct an empirical study to investigate whether converting CUTs to PUTs helps to find bugs and improve code coverage.
In addition, they propose a methodology to help developers in systematically retrofitting CUTs as PUTs.
Tsukamoto et al.~\cite{Tsukamoto18put} propose a fully automated CUT-PUT retrofitting technique called AutoPut, It is not parameterized for a single test case, it is for the test cases where there are multiple that can be parameterized. It first uses code clone detection techniques to detect duplicate test cases that can be merged from existing test cases in open source code. It then extracts and parameterizes multiple test cases that can be parameterized.
